Towards Functorial Language-Games

In categorical compositional semantics of natural language one studies functors from a category of grammatical derivations (such as a Lambek pregroup) to a semantic category (such as real vector spaces). We compositionally build game-theoretic semantics of sentences by taking the semantic category to be the category whose morphisms are open games. This requires some modifications to the grammar category to compensate for the failure of open games to form a compact closed category. We illustrate the theory using simple examples of Wittgenstein's language-games.

==> eptcsdata.tex <==
\providecommand{\firstpage}{89}
\providecommand{\publicationstatus}{B. Coecke, J. Hedges, D. Kartsaklis, M. Lewis, D. Marsden (Eds.):\\2018 Workshop on Compositional Approaches\\for Physics, NLP, and Social Sciences (CAPNS)\\
EPTCS 283, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.283.7}{10.4204/EPTCS.283.7}}

